Cross-Layer Deanonymization Methods in the Lightning Protocol

Bitcoin (BTC) pseudonyms (layer 1) can effectively be deanonymized using heuristic clustering techniques. However, while performing transactions off-chain (layer 2) in the Lightning Network (LN) seems to enhance privacy, a systematic analysis of the anonymity and privacy leakages due to the interaction between the two layers is missing. We present clustering heuristics that group BTC addresses, based on their interaction with the LN, as well as LN nodes, based on shared naming and hosting information. We also present linking heuristics that link 45.97% of all LN nodes to 29.61% BTC addresses interacting with the LN. These links allow us to attribute information (e.g., aliases, IP addresses) to 21.19% of the BTC addresses contributing to their deanonymization. Further, these deanonymization results suggest that the security and privacy of LN payments are weaker than commonly believed, with LN users being at the mercy of as few as five actors that control 36 nodes and over 33% of the total capacity. Overall, this is the first paper to present a method for linking LN nodes with BTC addresses across layers and to discuss privacy and security implications.

==> macros-generic.tex <==

%%Macros for the todos
\RequirePackage{color,colortbl}

\newcommand{\todoB}[1]{
\if\relax\detokenize{#1}\relax
    \textcolor{blue}{TODO}
  \else
    \textcolor{blue}{ \ifdraft {To Bernhard: #1} \fi}
  \fi
}

\newcommand{\todoF}[1]{
\if\relax\detokenize{#1}\relax
    \textcolor{green}{TODO}
  \else
    \textcolor{green}{ \ifdraft {To Friedhelm: #1} \fi}
  \fi
}

\newcommand{\todoMR}[1]{
\if\relax\detokenize{#1}\relax
    \textcolor{red}{TODO}
  \else
    \textcolor{red}{ \ifdraft {To Matteo Romiti: #1} \fi}
  \fi
}

\newcommand{\todoP}[1]{
  \if\relax\detokenize{#1}\relax
    \textcolor{orange}{TODO}
  \else
    \textcolor{orange}{ \ifdraft {To Pedro: #1}\fi}
  \fi
}

\newcommand{\todoMM}[1]{
  \if\relax\detokenize{#1}\relax
    \textcolor{brown}{TODO}
  \else
    \textcolor{brown}{ \ifdraft {To Matteo Maffei: #1}\fi}
  \fi
}

\newcommand{\todo}[1]{
\if\relax\detokenize{#1}\relax
    \textcolor{purple}{TODO}
  \else
    \textcolor{purple}{\ifdraft {#1}\fi}
  \fi
}




%%Macros for the term "heuristic/algorithm/function" to cluster entities or nodes
\newcommand{\algorithmcluster}{clustering algorithm\xspace}
\newcommand{\algorithmscluster}{clustering algorithms\xspace}
\newcommand{\Algorithmcluster}{Clustering Algorithm\xspace}
\newcommand{\Algorithmscluster}{Clustering algorithms\xspace}

%%Macros for the term "heuristic/algorithm/function" to link entities to nodes
\newcommand{\algorithmlink}{linking algorithm\xspace}
\newcommand{\algorithmslink}{linking algorithms\xspace}
\newcommand{\Algorithmlink}{Linking Algorithm\xspace}
\newcommand{\Algorithmslink}{Linking Algorithms\xspace}

%%Macros for theorem environments
%\newtheorem{definition}{Definition}


%%Macros for users
\newcommand{\usertext}{user\xspace}
\newcommand{\userstext}{users\xspace}
\newcommand{\Usertext}{User\xspace}
\newcommand{\Userstext}{Users\xspace}


%%Macros for entities
\newcommand{\entity}{entity\xspace}
\newcommand{\entities}{entities\xspace}
\newcommand{\Entity}{Entity\xspace}
\newcommand{\Entities}{Entities\xspace}
\newcommand{\entityid}{\ensuremath{e}\xspace}
\newcommand{\fundingentity}{funding \entity}
\newcommand{\closeentity}{settlement \entity}


%%Macros for the Bitcoin blockchain
\newcommand{\Bitcoin}{BTC\xspace}

\newcommand{\address}{address\xspace}
\newcommand{\addresses}{addresses\xspace}
\newcommand{\Address}{Address\xspace}
\newcommand{\Addresses}{Addresses\xspace}
\newcommand{\addressid}{a\xspace}

\newcommand{\fundingaddress}{funding address\xspace}
\newcommand{\fundingaddresses}{funding addresses\xspace}
\newcommand{\closeaddress}{settlement address\xspace}
\newcommand{\closeaddresses}{settlement addresses\xspace}
\newcommand{\channeladdress}{multisig address\xspace}


\newcommand{\txcond}{\ensuremath{\mathsf{cond}}\xspace}
\newcommand{\amt}{\ensuremath{\mathsf{cash}}\xspace}

\newcommand{\tx}{transaction\xspace}
\newcommand{\Tx}{Transaction\xspace}
\newcommand{\txs}{transactions\xspace}
\newcommand{\Txs}{Transactions\xspace}
\newcommand{\txid}{\ensuremath{\textit{tx}}\xspace}

\newcommand{\txidentifier}{\ensuremath{\mathsf{txid}}\xspace}
\newcommand{\txinput}{\ensuremath{\mathsf{Input}}\xspace}
\newcommand{\txoutput}{\ensuremath{\mathsf{Output}}\xspace}
\newcommand{\txwitness}{\ensuremath{\mathsf{Witness}}\xspace}

%%Macros for the LN
\newcommand{\LN}{LN\xspace}

\newcommand{\lMinusOne}{layer-1\xspace}
\newcommand{\lMinusTwo}{layer-2\xspace}

\newcommand{\lone}{layer 1\xspace}
\newcommand{\Lone}{Layer 1\xspace}
\newcommand{\ltwo}{layer 2\xspace}
\newcommand{\Ltwo}{Layer 2\xspace}

\newcommand{\node}{node\xspace}
\newcommand{\nodes}{nodes\xspace}
\newcommand{\Node}{Node\xspace}
\newcommand{\Nodes}{Nodes\xspace}

\newcommand{\nodeid}{\ensuremath{n}\xspace}

\newcommand{\pcid}{\textit{c}\xspace}

\newcommand{\nodeidentifier}{\ensuremath{\mathsf{nid}}\xspace}
\newcommand{\nodeip}{\ensuremath{\mathsf{IP}}\xspace}
\newcommand{\nodealias}{\ensuremath{\mathsf{Alias}}\xspace}

\newcommand{\channelOutputIndex}{\ensuremath{\mathsf{choutindex}}\xspace}
\newcommand{\chidentifier}{\ensuremath{\mathsf{chpoint}}\xspace}
\newcommand{\chbal}{\ensuremath{\mathsf{bal}}\xspace}
\newcommand{\balance}{\ensuremath{x}\xspace}
\newcommand{\chcap}{\ensuremath{\mathsf{cap}}\xspace}

%%Macros for transactions
\newcommand{\openchtx}{funding transaction\xspace}
\newcommand{\openchtxs}{funding transactions\xspace}
\newcommand{\closechtx}{settlement transaction\xspace}
\newcommand{\closechtxs}{settlement transactions\xspace}
\newcommand{\openchtxid}{\ensuremath{\txid_F}\xspace}
\newcommand{\closechtxid}{\ensuremath{\txid_S}\xspace}



%%Cryptographic operations
\newcommand{\hashfun}{\ensuremath{H}\xspace}
\newcommand{\pk}{\ensuremath{\textit{pk}}\xspace}
\newcommand{\set}[1]{\{#1\}\xspace}


%%Macros for data
\newcommand{\setnodesLN}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\setchannelsLN}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\setaddressbtc}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\settxs}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\setentities}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\collectionentities}{\ensuremath{\hat{E}}\xspace}
\newcommand{\setlinkedtuples}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\powerset}[1]{\ensuremath{\mathcal{P}(#1)}\xspace}


%%Macros for heuristic1
\newcommand{\setfundingentities}{\ensuremath{\setentities_F}\xspace}
\newcommand{\setsettlemententities}{\ensuremath{\setentities_S}\xspace}
\newcommand{\setfundingtxs}{\ensuremath{\settxs_F}\xspace}
\newcommand{\setsettlementtxs}{\ensuremath{\settxs_S}\xspace}
\newcommand{\setintersectionsymbol}{\ensuremath{\cap}\xspace}
\newcommand{\setcommonentities}{\ensuremath{\hat{\setentities}}\xspace}


%%Macros for heuristic2
\newcommand{\degreeentity}{\ensuremath{\textit{degEnt}}\xspace}
\newcommand{\degreenode}{\ensuremath{\textit{degNode}}\xspace}
\newcommand{\numberofchannels}{\ensuremath{N_C}\xspace}
\newcommand{\numberofchannelsmin}{\ensuremath{deg_{min}}\xspace}


%%%Macros for evaluation
\newcommand{\minMinConf}{\ensuremath{2}\xspace}
\newcommand{\maxMinConf}{\ensuremath{10}\xspace}

\newcommand{\nAddressesFundingSettling}{\ensuremath{238,070}\xspace}
\newcommand{\nAddressesGS}{\ensuremath{703,443,739}\xspace}
\newcommand{\nAddressesAliasIPTagged}{\ensuremath{50,456}\xspace}
\newcommand{\nAddressesAliasTagged}{\ensuremath{50,157}\xspace}
\newcommand{\nAddressesIPTagged}{\ensuremath{48,739}\xspace}

\newcommand{\nAddressesStar}{\ensuremath{144}\xspace}
\newcommand{\nAddressesSnake}{\ensuremath{18,556}\xspace}
\newcommand{\nAddressesCollector}{\ensuremath{6,146}\xspace}
\newcommand{\nAddressesProxy}{\ensuremath{12,292}\xspace}
\newcommand{\percAddressesStar}{\ensuremath{0.0}}
\newcommand{\percAddressesSnake}{\ensuremath{0.0}}
\newcommand{\percAddressesCollector}{\ensuremath{0.0}}
\newcommand{\percAddressesProxy}{\ensuremath{0.0}}

\newcommand{\nBTCNow}{\ensuremath{1,108.70}\xspace}
\newcommand{\nBlocks}{\ensuremath{647,529}\xspace}
\newcommand{\nChannelsOpen}{\ensuremath{37,996}\xspace}
\newcommand{\nChannelsNow}{\ensuremath{37,003}\xspace}
\newcommand{\nChannelsUsed}{\ensuremath{98,431}\xspace}
\newcommand{\nClustersOffChainOnly}{\ensuremath{301}\xspace}
\newcommand{\nEntitiesFundingSettling}{\ensuremath{138,457}\xspace}
\newcommand{\nEntitiesFunding}{\ensuremath{96,181}\xspace}
\newcommand{\nEntitiesGS}{\ensuremath{336,847,691}\xspace}
\newcommand{\nEntitiesReusedHeurOneNone}{\ensuremath{22}\xspace}
\newcommand{\nEntitiesTwoOutputsNone}{\ensuremath{32,321}\xspace}

\newcommand{\nEntitiesStar}{\ensuremath{139}\xspace} 
\newcommand{\nEntitiesSnake}{\ensuremath{18,512}\xspace} 
\newcommand{\nEntitiesCollector}{\ensuremath{3,923}\xspace} 
\newcommand{\nEntitiesProxy}{\ensuremath{3,229}\xspace} 
\newcommand{\percEntitiesStar}{\ensuremath{0.0}} 
\newcommand{\percEntitiesSnake}{\ensuremath{19}} 
\newcommand{\percEntitiesCollector}{\ensuremath{7}} 
\newcommand{\percEntitiesProxy}{\ensuremath{6}} 

\newcommand{\nEntitiesSource}{\ensuremath{196,131}\xspace} 
\newcommand{\nEntitiesDestination}{\ensuremath{424,732}\xspace} 

\newcommand{\nEntitiesLinkedHeurOneNone}{\ensuremath{9,042}\xspace}
\newcommand{\nEntitiesLinkedHeurOneAll}{\ensuremath{11,272}\xspace}

\newcommand{\nEntitiesLinkedHeurTwoMinConfNone}{\ensuremath{9,904}\xspace}
\newcommand{\nEntitiesLinkedHeurTwoMinConfAll}{\ensuremath{17,606}\xspace}

\newcommand{\nEntitiesSettlement}{\ensuremath{53,370}\xspace}

\newcommand{\nEntitiesAliasIPTagged}{\ensuremath{17,260}\xspace}
\newcommand{\nEntitiesAliasTagged}{\ensuremath{17,135}\xspace}
\newcommand{\nEntitiesIPTagged}{\ensuremath{16545}\xspace}

\newcommand{\nNodesInChannels}{\ensuremath{10,910}\xspace}

\newcommand{\nNodesLinkedHeurOneNone}{\ensuremath{2,170}\xspace}
\newcommand{\nNodesLinkedHeurOneAll}{\ensuremath{2,579}\xspace}

\newcommand{\nNodesLinkedHeurTwoAll}{\ensuremath{2579}\xspace}
\newcommand{\nNodesLinkedHeurTwoMinConfNone}{\ensuremath{2,170}\xspace}
\newcommand{\nNodesNow}{\ensuremath{13,902}\xspace}
\newcommand{\nNodesTwoOutputs}{\ensuremath{4,621}\xspace}

\newcommand{\nNodesLinkedWithAlias}{\ensuremath{4,284}\xspace}
\newcommand{\nNodesLinkedWithIP}{\ensuremath{3,919}\xspace}
\newcommand{\nNodesAliasIPCluster}{\ensuremath{1,251}\xspace}
\newcommand{\nNodesLinkedAliasIPClusterHeurOne}{\ensuremath{310}\xspace}
\newcommand{\nNodesLinkedAliasIPClusterHeurTwo}{\ensuremath{416}\xspace}
\newcommand{\nNodesAliasIPLinkableHeurOne}{\ensuremath{259}\xspace}
\newcommand{\nNodesAliasIPLinkableHeurTwo}{\ensuremath{245}\xspace}

\newcommand{\nLinksReusedHeurOne}{\ensuremath{83}\xspace}
\newcommand{\nPaths}{\ensuremath{23,829,202}\xspace}

\newcommand{\nStars}{\ensuremath{52}\xspace}
\newcommand{\nSnakes}{\ensuremath{5,638}\xspace}
\newcommand{\nCollectors}{\ensuremath{1,476}\xspace}
\newcommand{\nProxies}{\ensuremath{989}\xspace}
\newcommand{\nComponentsFundingRelevant}{\ensuremath{18,407}\xspace}
\newcommand{\nComponentsSettlementRelevant}{\ensuremath{10,750}\xspace}
\newcommand{\percStars}{\ensuremath{0.3}}
\newcommand{\percSnakes}{\ensuremath{31}}
\newcommand{\percCollectors}{\ensuremath{14}}
\newcommand{\percProxies}{\ensuremath{9}}
\newcommand{\percCollectorsProxies}{\ensuremath{23}}

\newcommand{\nTxsFunding}{\ensuremath{98,240}\xspace}
\newcommand{\nTxsFundingSettling}{\ensuremath{158,687}\xspace}
\newcommand{\nTxsClosing}{\ensuremath{60,447}\xspace}
\newcommand{\nTxsClosingTwoOutputs}{\ensuremath{25,686}\xspace}
\newcommand{\nTxsGS}{\ensuremath{566,776,778}\xspace}
\newcommand{\nUSDNow}{\ensuremath{11,569,618}\xspace}

\newcommand{\percAddressesLinkedHeurOneNone}{\ensuremath{18.16}}
\newcommand{\percAddressesLinkedHeurOneStar}{\ensuremath{18.16}}
\newcommand{\percAddressesLinkedHeurOneSnake}{\ensuremath{18.18}}
\newcommand{\percAddressesLinkedHeurOneCollector}{\ensuremath{18.36}}
\newcommand{\percAddressesLinkedHeurOneProxy}{\ensuremath{20.12}}
\newcommand{\percAddressesLinkedHeurOneAll}{\ensuremath{20.96}}

\newcommand{\percAddressesLinkedHeurTwoMinConfNone}{\ensuremath{19.19}}
\newcommand{\percAddressesLinkedHeurTwoMinConfStar}{\ensuremath{19.22}}
\newcommand{\percAddressesLinkedHeurTwoMinConfSnake}{\ensuremath{26.8}}
\newcommand{\percAddressesLinkedHeurTwoMinConfCollector}{\ensuremath{19.39}}
\newcommand{\percAddressesLinkedHeurTwoMinConfProxy}{\ensuremath{21.16}}
\newcommand{\percAddressesLinkedHeurTwoMinConfAll}{\ensuremath{29.61}}

\newcommand{\percEntitiesLinkedHeurOneNone}{\ensuremath{6.53}}
\newcommand{\percEntitiesLinkedHeurOneStar}{\ensuremath{6.53}}
\newcommand{\percEntitiesLinkedHeurOneSnake}{\ensuremath{6.53}}
\newcommand{\percEntitiesLinkedHeurOneCollector}{\ensuremath{6.64}}
\newcommand{\percEntitiesLinkedHeurOneProxy}{\ensuremath{7.64}}
\newcommand{\percEntitiesLinkedHeurOneAll}{\ensuremath{8.14}}

\newcommand{\percEntitiesLinkedHeurOneTwoOutputsNone}{\ensuremath{27.98}}

\newcommand{\percEntitiesLinkedHeurTwoMinConfNone}{\ensuremath{7.15}}
\newcommand{\percEntitiesLinkedHeurTwoMinConfStar}{\ensuremath{7.17}}
\newcommand{\percEntitiesLinkedHeurTwoMinConfSnake}{\ensuremath{11.09}}
\newcommand{\percEntitiesLinkedHeurTwoMinConfCollector}{\ensuremath{7.26}}
\newcommand{\percEntitiesLinkedHeurTwoMinConfProxy}{\ensuremath{8.27}}
\newcommand{\percEntitiesLinkedHeurTwoMinConfAll}{\ensuremath{12.72}}

% sum of starsnake entities /total funding entities
% () / 
\newcommand{\percEntitiesFundingClustered}{\ensuremath{19.39}}
% sum of collproxy entities /total settlement entities
\newcommand{\percEntitiesSettlementClustered}{\ensuremath{13.40}}
% sum of starsnake entities
\newcommand{\nEntitiesFundingClustered}{\ensuremath{18,651}\xspace}
% sum of collproxy entities
\newcommand{\nEntitiesSettlementClustered}{\ensuremath{7,152}\xspace}
% sum of starsnake addresses
\newcommand{\nAddressesFundingClustered}{\ensuremath{18,700}\xspace}
% sum of collproxy addresses
\newcommand{\nAddressesSettlementClustered}{\ensuremath{18,438}\xspace}

\newcommand{\percNodesLinkedHeurOneNone}{\ensuremath{19.89}}
\newcommand{\percNodesLinkedHeurOneStar}{\ensuremath{19.89}}
\newcommand{\percNodesLinkedHeurOneSnake}{\ensuremath{19.89}}
\newcommand{\percNodesLinkedHeurOneCollector}{\ensuremath{19.97}}
\newcommand{\percNodesLinkedHeurOneProxy}{\ensuremath{22.81}}
\newcommand{\percNodesLinkedHeurOneAll}{\ensuremath{23.64}}
% percNodesLinkedHeurOneAll + percNodesLinkedAliasIPClusterHeurOne
\newcommand{\percNodesLinkedHeurOneAllAliasIP}{\ensuremath{26.48}}

\newcommand{\percNodesLinkedHeurOneTwoOutputsNone}{\ensuremath{46.91}}

\newcommand{\percNodesLinkedHeurTwoMinConfNone}{\ensuremath{22.84}}
\newcommand{\percNodesLinkedHeurTwoMinConfStar}{\ensuremath{22.96}}
\newcommand{\percNodesLinkedHeurTwoMinConfSnake}{\ensuremath{39.84}}
\newcommand{\percNodesLinkedHeurTwoMinConfCollector}{\ensuremath{22.97}}
\newcommand{\percNodesLinkedHeurTwoMinConfProxy}{\ensuremath{25.6}}
\newcommand{\percNodesLinkedHeurTwoMinConfAll}{\ensuremath{42.16}}
% percNodesLinkedHeurTwoMinConfAll + percNodesLinkedAliasIPClusterHeurTwo
\newcommand{\percNodesLinkedHeurTwoMinConfAllAliasIP}{\ensuremath{45.97}}

% nNodesLinkedAliasIPClusterHeurTwo/nNodesInChannels
\newcommand{\percNodesLinkedAliasIPClusterHeurTwo}{\ensuremath{3.81}} 
\newcommand{\percNodesLinkedAliasIPClusterHeurOne}{\ensuremath{2.84}} 
% nAddressesAliasIPTagged/nAddressesFundingSettling
\newcommand{\percAddressesAliasIPTagged}{\ensuremath{21.19}}

\newcommand{\percTxSettlementOneOutput}{\ensuremath{56.3}}
\newcommand{\percTxSettlementTwoOutputs}{\ensuremath{41.8}} 
\newcommand{\percTxSettlementMoreThanTwoOutputs}{\ensuremath{1.9}} 

%%%%%%% Validation %%%%%%%
\newcommand{\nNodesOpenedChannelsToUs}{\ensuremath{3}\xspace}
\newcommand{\nNodesOpenedChannelsToUsValidated}{\ensuremath{2}\xspace}
\newcommand{\nChannelsWeOpenedAndClosed}{\ensuremath{81}\xspace}
\newcommand{\nNodesWeClosedChannelWith}{\ensuremath{73}\xspace}
\newcommand{\nNodesReceivedOurCoins}{\ensuremath{52}\xspace}
\newcommand{\nNodesReceivedSpentOurCoins}{\ensuremath{11}\xspace}
\newcommand{\nNodesReceivedSpentOurCoinsValidates}{\ensuremath{7}\xspace}
\newcommand{\nNodesReceivedOurCoinsLinked}{\ensuremath{52}\xspace}
\newcommand{\nNodesReceivedOurCoinsNewAddressUnspent}{\ensuremath{41}\xspace}
\newcommand{\nNodesValidated}{\ensuremath{9}\xspace} 
\newcommand{\nSettlementTxsWithTwoOutputs}{\ensuremath{58}\xspace} 

%%Macros for graph
\newcommand{\GG}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\VV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\EE}{\ensuremath{\mathcal{E}}\xspace}


%%%Macros for tables
\definecolor{Gray}{gray}{0.9}

